DRAMScope: Uncovering DRAM Microarchitecture and Characteristics by Issuing Memory Commands

The demand for precise information on DRAM microarchitectures and error characteristics has surged, driven by the need to explore processing in memory, enhance reliability, and mitigate security vulnerability. Nonetheless, DRAM manufacturers have disclosed only a limited amount of information, making it difficult to find specific information on their DRAM microarchitectures. This paper addresses this gap by presenting more rigorous findings on the microarchitectures of commodity DRAM chips and their impacts on the characteristics of activate-induced bitflips (AIBs), such as RowHammer and RowPress. The previous studies have also attempted to understand the DRAM microarchitectures and associated behaviors, but we have found some of their results to be misled by inaccurate address mapping and internal data swizzling, or lack of a deeper understanding of the modern DRAM cell structure. For accurate and efficient reverse-engineering, we use three tools: AIBs, retention time test, and RowCopy, which can be cross-validated. With these three tools, we first take a macroscopic view of modern DRAM chips to uncover the size, structure, and operation of their subarrays, memory array tiles (MATs), and rows. Then, we analyze AIB characteristics based on the microscopic view of the DRAM microarchitecture, such as 6F^2 cell layout, through which we rectify misunderstandings regarding AIBs and discover a new data pattern that accelerates AIBs. Lastly, based on our findings at both macroscopic and microscopic levels, we identify previously unknown AIB vulnerabilities and propose a simple yet effective protection solution.

==> 0_cover_page.tex <==
%\section{0_cover_page}
\label{sec:0_cover_page}

We appreciate the reviewers' constructive comments. 
%
Below, we address each reviewer's comments. 
%
Click on the blue hyperlink, such as `A-1' to jump to the corresponding section.
%
%We color the revised parts of the manuscript in blue.
%

\noindent
\rule[0.5ex]{8.8cm}{0.5pt}

\noindent
\textbf{[\#A-1] Novelty of our observations}
%

To the best of our knowledge, our observations are either verified for the first time despite some prior assumptions \textbf{(O1/2/4/5)} or identified for the first time \textbf{(O3/6/7/8/9/10/11/12/13/14)}. 
%
Two observations \textbf{(O11/12)} even contradict the prior findings, which fall into three common pitfalls (\rev{\S\ref{sec:3-3_common_pitfalls}}) in complex address remapping. 
%
Throughout our observations, we comprehensively uncover and clarify certain details of DRAM internal structures (e.g., data swizzling, edge subarrays, MAT size, and coupled rows) of various DRAM chips. 
%
Also, we analyze the influence of horizontally adjacent cells’ charge, i.e., vertical effects, on AIB characteristics.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
\rule[0.5ex]{8.8cm}{0.5pt}

\noindent
\textbf{[\#D-1, 2, 3] Details of experimental methodology and configurations}
%

First, we clarified the DRAM chips we tested and added \rev{Table~\ref{tbl:3_tested_chips}}, which shows the distribution of the tested DRAM chips. 
%
Second, we revised the texts regarding the details of the uncovered subarray heights in \rev{Table~\ref{tbl:4_contribution1}}. 
%
Lastly, we clarified that we observe consistent experimental results across different tested DRAM chips in \rev{\hyperref[review_D-1]{D-1}, {\hyperref[review_D-2]{D-2}, and \hyperref[review_D-3]{D-3} (\S\ref{sec:4_contribution1})}}. 
%
Also, we mentioned that we did not observe any clear discrepancies when a wider range of rows and banks were tested. 
%
Prior works~\cite{isca-2020-revisit, arxiv-2023-hbm2_rowhammer, micro-2021-deeper} also sampled 1K rows in analyzing RowHammer characterization.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
\rule[0.5ex]{8.8cm}{0.5pt}

\noindent
\textbf{[\#D-4] Possible limitations of our observations}
%

First, we additionally conducted experiments for $\times$8 chips, where we did not observe any significant disparity \rev{(\S\ref{sec:4_contribution1} and \S\ref{sec:5_contribution2})}. 
%
Second, the utilized Xilinx Alveo U200 and U280 only support up to DDR4 1.6 Gbps, and U280 is fixed with HBM2 1.2 Gbps. 
%
However, the wall-clock times of various relevant timing parameters (e.g., tRAS, tRP, and tRC) are only marginally affected by the DRAM frequency. 
%
Thus, even if the tested DRAM frequency changes with a different FPGA device, we do not expect to see a discrepancy in the observed AIB characteristics.
%
We discussed this in \rev{\hyperref[review_D-4]{D-4} (\S\ref{sec:3-1_fpga_environment})}.

\noindent
\rule[0.5ex]{8.8cm}{0.5pt}

\noindent
\textbf{[\#E-1] Implications of memory encryption}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We added corresponding discussions in \rev{\hyperref[review_E-1]{E-1} (\S\ref{sec:6_vuln_prot})}. 
%
We agree that adopting memory encryption technologies (e.g., AMD memory encryption) can also thwart the data pattern-aware AIB attacks. 
%
We argue that the originally mentioned simple masking technique, which does not necessarily encrypt the data, can achieve a similar effect against AIB attacks yet with a lower performance/energy/area overhead.

\noindent
\rule[0.5ex]{8.8cm}{0.5pt}

\noindent
\textbf{[\#B-1, 2, 3] Correlation with two failure mechanisms of AIB}
%

We added the suggested references~\cite{iedm-2017-reliability,ted-2021-physics} and revised \rev{\hyperref[review_B-1]{B-1} (\S\ref{subsec:2_4_activate-induced_bitflips}), \hyperref[review_B-2]{B-2} (\S\ref{sec:3-2_reverse_techniques}), and \hyperref[review_B-3]{B-3}
(\S\ref{sec:5-2_aib_characteristics})} with further details on failure mechanisms. 
%
We believe that our microscopic findings are a direct influence of two types of failure mechanisms. 
%
However, we avoided specifying each gate’s type as neighboring gate (NG) or passing gate (PG) by linking it to failure mechanisms, due to uncertainties in RowPress experimental results. 
%
RowHammer can accelerate charge injection (1$\rightarrow$0) from NG and capacitive crosstalk (0$\rightarrow$1) from PG~\cite{iedm-2017-reliability,ted-2021-physics}. %[55, 68]. 
%
Based on this, in Figure~\ref{fig:6f2_graph}(e)(f) depicting the upper aggressor, we can conjecture that the blue odd-bit cells (orange even-bit cells) are caused by activating PG (NG). 
%
However, the failure mechanism of RowPress is not well studied, except for a brief mention in an arXiv paper~\cite{arxiv-2023-dsac}. 
%
Our findings misalign with that. 
%
In Figure~\ref{fig:6f2_graph}(a)(b) depicting the upper aggressor, orange even-bit cells that are conjectured to form NG also demonstrate charge injection (1$\rightarrow$0) from RowPress, contradicting prior work~\cite{arxiv-2023-dsac}.

\noindent
\rule[0.5ex]{8.8cm}{0.5pt}

\noindent
\textbf{[\#C-1] AIB characteristics across HBM stacks and the impact of aging}
%

Although such a finding would be highly interesting, across-stack interference is less likely to occur due to the large stack-to-stack distance. 
%
According to a recent study [\hyperref[R1]{R1}], SK Hynix’s HBM3 uses a 1z-nm process with an approximately 30-um thick HBM core die. 
%
Electromagnetic interference, which causes AIBs, scales inverse-quadratically by distance. 
%
Considering that we did not observe any AIB phenomenon even between two adjacent subarrays (100 times the cell-to-cell distance~\cite{rambus-dram}) as in~\cite{sosp-2023-siloz,arxiv-2023-hbm2_rowhammer}, stack-to-stack influence is likely to be negligible. 
%
We also could not recognize any impact of aging on AIB characteristics among the tested DRAM chips. 
%
This aligns with prior studies reporting that aging has no clear impact on any type of DRAM fault rates~\cite{isca-2020-revisit,dft-2017-lifetime}. 
%
Accordingly, we newly clarified in \rev{\hyperref[review_C-1]{C-1} (\S\ref{sec:3-1_fpga_environment})} that we do not consider aging impact in our study.

\noindent
\rule[0.5ex]{8.8cm}{0.5pt}

\noindent
\textbf{[\#A/E-1, 2, 3] Implications of our observations in AIB attack/defense and PIM architecture}
%

We have augmented \rev{\hyperref[review_A/E-1]{A/E-1}, \hyperref[review_A/E-2]{A/E-2}, and \hyperref[review_A/E-3]{A/E-3} (\S\ref{sec:6_vuln_prot})}, which discuss the impact of our findings on the AIB attack/defense and PIM architecture. 
%
First, we added another attack scenario that exploits the coupled row to circumvent the counter-based AIB protection solutions, and a potential patch as a solution. 
%
We also discussed the recently introduced DRFM interface, where the MC provides a specific target address. 
%
We argue that even the coupled row structure does not undermine DRFM because the adjacent rows of the given target row are calculated at the DRAM side~\cite{jedec-ddr4,jedec-ddr5}. 
%
Lastly, we newly discuss the impact of our findings on the reliability of certain PIM architectures.

\noindent
\rule[0.5ex]{8.8cm}{0.5pt}

\noindent
\textbf{Reference}

\noindent
\label{R1}
[R1] M. -J. Park et al., ``A 192-Gb 12-High 896-GB/s HBM3 DRAM With a TSV Auto-Calibration Scheme and Machine-Learning-Based Layout Optimization,'' in IEEE Journal of Solid-State Circuits, vol. 58, no. 1, pp. 256-269, 2023.

